Data-Pooling in Stochastic Optimization

Managing large-scale systems often involves simultaneously solving thousands of unrelated stochastic optimization problems, each with limited data. Intuition suggests one can decouple these unrelated problems and solve them separately without loss of generality. We propose a novel data-pooling algorithm called Shrunken-SAA that disproves this intuition. In particular, we prove that combining data across problems can outperform decoupling, even when there is no a priori structure linking the problems and data are drawn independently. Our approach does not require strong distributional assumptions and applies to constrained, possibly non-convex, non-smooth optimization problems such as vehicle-routing, economic lot-sizing or facility location. We compare and contrast our results to a similar phenomenon in statistics (Stein's Phenomenon), highlighting unique features that arise in the optimization setting that are not present in estimation. We further prove that as the number of problems grows large, Shrunken-SAA learns if pooling can improve upon decoupling and the optimal amount to pool, even if the average amount of data per problem is fixed and bounded. Importantly, we highlight a simple intuition based on stability that highlights when and why data-pooling offers a benefit, elucidating this perhaps surprising phenomenon. This intuition further suggests that data-pooling offers the most benefits when there are many problems, each of which has a small amount of relevant data. Finally, we demonstrate the practical benefits of data-pooling using real data from a chain of retail drug stores in the context of inventory management.

==> 10_E_OmittedProofsLargeSample_Smooth.tex <==
%!TEX root = 0_main_DataPooling.tex

\newpage
{\blockedit
\section{Performance in the Large-Sample Limit}
\label{sec:LargeSampleSmooth}

In this section, we prove that for any anchor $h(\bfmhat)$, $\bx_k(\alphaLOO_h, h(\bfmhat), \bfmhat_k)$ performs comparably to the full-information optimum solution $\bx_k^*$ in a large-sample limit, i.e., $K$ fixed and $N \rightarrow \infty$.  The key idea is to show that 
$\bx_k(\alphaLOO_h, h(\bfmhat), \bfmhat_k)$ approximately optimizes the SAA objective, and, since the SAA objective converges to the true objective in this limit, 
that $\bx_k(\alphaLOO_h, h(\bfmhat), \bfmhat_k)$ performs comparably to the full-information optimum.  

First recall the definitions of $\Zperf$ and $\Zloo$, 
\begin{align*}
\Zperf(\alpha, \bq) \equiv \frac{1}{K} \sum_{k=1}^K Z_k(\alpha, \bq), 
\quad &\text{ where } \quad Z_k(\alpha, \bq) \equiv \frac{\lambda_k}{\lambdabar} \bp_k^\top \bc_k(\bx_k(\alpha, \bq, \bfmhat_k) ) 
\\
\Zloo(\alpha, \bq) \equiv \frac{1}{K} \sum_{k=1}^K Z^{\sf LOO}(\alpha, \bq), 
\quad &\text{ where } \quad Z_k^{\sf LOO}(\alpha, \bq) \equiv \frac{1}{N \lambdabar} \sum_{i=1}^d \mhat_{ki} c_{ki}(\bx_k(\alpha, \bq, \bfmhat_k - \be_i) ).
\end{align*}
Furthermore, recall the full-information solutions $\bx_k^* \in \argmin_{\bx \in \X_k} \frac{\lambda_k}{\lambdabar} \bp_k^\top \bc_k(\bx)$, with performances
\begin{align*}
\overline Z_K^* \equiv \frac{1}{K} \sum_{k=1}^K Z^*_k, 
\quad &\text{ where } \quad Z^*_k \equiv \frac{\lambda_k}{\lambdabar}  \bp_k^\top \bc_k(\bx_k^* ).
\end{align*}
Analogously, we next define, 
\[
\ZSAA(\alpha, \bp_0) \equiv \frac{1}{K} \sum_{k=1}^K Z^{\sf SAA}_k(\alpha, \bp_0), 
\quad \text{ where } \quad
Z^{\sf SAA}_k(\alpha, \bp_0) \equiv \frac{1}{N \lambdabar} \bfmhat_k^\top \bc_k(\bx_k(\alpha, \bp_0, \bfmhat_k)).
\]
In words, $Z^{\sf SAA}_k(\alpha, \bp_0)$ measures the in-sample performance of the policy $\bx_k(\alpha, \bp_0, \bfmhat_k)$.  

In what follows, we will also require the following lemma on the tail of a Poisson random variable.  

\begin{lemma}[Poisson Concentration]  \label{lem:PoissonConcentration}
Suppose $\Nhat_k \sim \text{Poisson}(N_k)$.  For any $\delta > 0$ such that $3\log(2/\delta) < N_k$,  we have with probability at least $1-\delta$ that 
\(
\abs{ \Nhat_k - N_k} \leq \sqrt{3 N_k \log( 2/ \delta)}.
\)
\end{lemma}
\proof{Proof.}
From a Chernoff-style argument for the tail of a Poisson random variable, we have for $t > 0$, 
\[
\P\left( \Nhat_k - N_k > t N_k \right)
\ = \ 
\P\left( \Nhat_k > (1+t) N_k \right)
 \ \leq \ \exp\left( - N_k ( (1+t) \log(1+t) - t) \right), 
\]
Similarly, when $-1 < t < 0$, a similar argument yields
\[
\P\left( N_k - \Nhat_k > t N_k \right) 
\ = \ 
\P\left( \Nhat_k < (1-t) N_k \right) 
\ \leq \ 
\exp \left( - N_k ( (1-t) \log(1-t) - t) \right).
\]
For $t \in [-1, 1]$, we have $(1+t) \log(1+t) - t \geq t^2/3$.  Hence, weakening both bounds to $\exp(-N_k t^2/3)$ and combining shows for $0 < t < 1$, $\P\left( \abs{\Nhat_k - N_k } > t N_k \right) \leq 2\exp(-N_k t^2/3)$.  Let $t = \sqrt{\frac{3\log(2/\delta)}{N_k}}$ to complete the proof.  
\endproof


Now, the first step of our proof formalizes the idea that $\alpha = 0$ optimizes the SAA performance.
\begin{lemma}[SAA Optimizes In-Sample Performance] \label{lem:SAAOptimizeInsample}
For any $\bp_0 \in \Delta_d$, 
\[
0 \in \arg\min_{\alpha \geq 0} \quad \ZSAA(\alpha, \bp_0).
\]
\end{lemma}
\proof{Proof.}  
We will show that $0 \in \arg \min_{\alpha \geq 0} Z_k^{\sf SAA}(\alpha, \bp_0)$ for each $k$, which implies the lemma.  
By definition of $\bx_k(0, \bp_0, \bfmhat_k)$ as an optimizer, 
\[
\frac{1}{\Nhat_k } \bfmhat_k^\top \bc(\bx_k(0, \bp_0, \bfmhat_k) )
\leq 
\frac{1}{\Nhat_k } \bfmhat_k^\top \bc(\bx) \quad \forall \bx \in \mathcal X_k. 
\]
Moreover, $\bx_k(\alpha, \bp_0, \bfmhat_k) \in \mathcal X_k$ for all $\alpha \geq 0$.  Thus, $Z_k^{\sf SAA}(0, \bp_0) \leq Z_k^{\sf SAA}(\alpha, \bp_0)$ for all $\alpha \geq 0$, completing the lemma.  
 \endproof

%


In the remainder, we focus on the case of Lipschitz, strong-convex problems.  The key intuition in this case can readily be adapted to other classes of problems.   

\subsection{Performance Guarantees for Strongly-Convex Problems in a Large-Sample Limit}
We first bound the difference between the leave-one-out performance and in-sample performance.  
\begin{lemma}[Relating LOO and SAA Performance] \label{lem:LOOToSAA}
Under the assumptions of \cref{thm:FixedPointShrinkage}, 
\[
\sup_{\alpha \geq 0, \bq \in \Delta_d} \abs{ \ZSAA(\alpha, \bp_0) - \Zloo(\alpha, \bq) } 
\ \leq  \  \frac{4L^2}{\gamma N\lambdabar}.
\]
Consequently, 
\[
0 \leq \ZSAA(\alphaLOO_h, h(\bfmhat_k)) - \ZSAA(0, h(\bfmhat_k)) \leq \frac{8L^2}{\gamma N\lambdabar}.
\]
\end{lemma}
\proof{Proof.}
Fix any $k$. If $\Nhat_k \geq 1$, then 
\begin{align*} \hspace{-20pt}
\abs{ Z^{\sf SAA}_k(\alpha, \bq) - Z^{\sf LOO}_k(\alpha, \bq) } 
&\   \leq \ 
\frac{1}{N \lambdabar} \sum_{i=1}^d \mhat_{ki} \abs{ c_{ki}(\bx_k(\alpha, \bq, \bfmhat_k)) - c_{ki}(\bx_k(\alpha, \bq, \bfmhat_k - \be_i)) }
\\
& \ \leq \ 
\frac{L}{N \lambdabar} \sum_{i=1}^d \mhat_{ki} \| \bx_k(\alpha, \bq, \bfmhat_k) - \bx_k(\alpha, \bq, \bfmhat_k - \be_i) \|_2 && (c_{ki}(\cdot) \text{ is $L$-Lipschitz})
\\
\\ 
& \ \leq \ 
\frac{4L^2 \Nhat_k}{N \lambdabar \gamma} && \text{(\cref{lem:ContinuityAlpha}, part~\ref{part:contLOO})}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\end{align*}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
On the other hand, if $\Nhat_k = 0$, then we have $\bfmhat_k = \bm 0$ and  $Z^{\sf SAA}_k(\alpha, \bq) = Z^{\sf LOO}_k(\alpha, \bq) = 0$. 

Combining, we have
$$
\abs{ Z^{\sf SAA}_k(\alpha, \bq) - Z^{\sf LOO}_k(\alpha, \bq) }\leq \frac{4L^2}{\gamma N\lambdabar}\indic{\Nhat_k\geq1}\leq \frac{4L^2}{\gamma N\lambdabar}.
$$
Thus, averaging over $k$, shows
\begin{align*}
\sup_{\alpha \geq 0, \bq \in \Delta_d} \abs{ \ZSAA(\alpha, \bp_0) - \Zloo(\alpha, \bq) }
&\  \leq \ \frac{4L^2}{\gamma N\lambdabar}.
\end{align*}
This proves the first statement of the lemma.

To complete the lemma, note the first inequality in the second statement follows from  \cref{lem:SAAOptimizeInsample}.  For the second inequality, write, 
\begin{align*}
\ZSAA\big(\alphaLOO_h, h(\bfmhat)\big) - \ZSAA\big(0, h(\bfmhat)\big)
& \  \leq \ 
\ZSAA\big(\alphaLOO_h, h(\bfmhat)\big) - \Zloo\big(\alphaLOO_h, h(\bfmhat)  \big)
\\ &\quad \ + \ 
\Zloo\big(\alphaLOO_h, h(\bfmhat)  \big) - \Zloo\big(0, h(\bfmhat)  \big) 
\\ &\quad \ + \ 
\Zloo(\big(0, h(\bfmhat)  \big)  - \ZSAA\big(0, h(\bfmhat)\big)
\\
&\  \leq\ 
2 \sup_{\alpha \geq 0, \bq \in \Delta_d} \abs{ \ZSAA\big(\alpha, \bq \big) - \Zloo\big(\alpha, \bq \big) }, 
\end{align*}
where the last inequality follows because 
\(
\Zloo\big(\alphaLOO_h, h(\bfmhat)  \big) \leq \Zloo\big(0, h(\bfmhat)  \big)
\)
by optimality of $\alphaLOO_h$.  Bound the supremum by the first result in the lemma to complete the proof.
\endproof

\Cref{lem:LOOToSAA} shows that the solutions $\bx_k(\alphaLOO_h, h(\bfmhat), \bfmhat_k)$ are, on average, at most $O_p(N^{-1})$ suboptimal in the SAA problem, as $N \rightarrow \infty$.  There are many classical (asymptotic) results relating approximate solutions to the SAA problem to the full-information optimal solution in the large-sample regime.  (See, e.g., \citealp[Chapter 5]{van2000asymptotic})  These results can be applied (conditional on $\bm \Nhat$) to obtain corresponding asymptotic results above. 

 To obtain finite-sample results, however, we need to slightly modify these classical arguments and account for the randomness in $\bm \Nhat$.  The remainder of the proof describes these modifications to the standard argument.  
%
\begin{comment}
We first have a simple concentration of the SAA performance of the optimal solution to the full-information performance. The assumption of bounded optimal costs is similar in flavor to \cref{asn:bounded}, and holds when, e.g., the functions $c_k(\cdot, \cdot)$ are uniformly bounded.  
\begin{lemma}[SAA Performance of $\bx_k^*$] \label{lem:SAAFullInfoConcentrates}
Assume that for each $k$, $\abs{ c_k(\bx^*_k, \bxi_k) } \leq \Cmax$.  For any $2K e^{-N \lambda_{\min} / 3} < \delta < \frac{1}{2}$, 
we have with probability at least $1-\delta$, 
\[
	\abs{\frac{1}{K}\sum_{k=1}^K \frac{\Nhat_k}{N \lambdabar} \bphat_k ^\top \bc_k(\bx^*_k) - \overline Z_K^*}  \ \leq \ 
	\frac{6 \Cmax  \sqrt{\log(K/\delta)  } }{\sqrt{ N \lambdabar}}     \ + \ 
	\frac{9\Cmax  \log(K/\delta)} { N \lambdabar}.
\]
\end{lemma}
\proof{Proof.}
Consider the $k^\text{th}$ element of the sum.  By triangle inequality and definition of $Z^*_k$, 
\begin{align*}
\abs{\frac{\Nhat_k}{N \lambdabar} \bphat_k ^\top \bc_k(\bx^*_k) -  Z^*_k} 
\ \leq \ 
\abs{\frac{\Nhat_k}{N \lambdabar} (\bphat_k - \bp_k)^\top \bc_k(\bx^*_k) } 
+ 
\abs{\left(\frac{\Nhat_k}{N \lambdabar} - \frac{N_k}{N \lambdabar} \right)\bp_k ^\top \bc_k(\bx^*_k)}. 
\end{align*}
We analyze each term separately.  

For the first term, if $\Nhat_k = 0$, the term equals $0$.  Otherwise, write
\[
\abs{\frac{\Nhat_k}{N \lambdabar} (\bphat_k - \bp_k)^\top \bc_k(\bx^*_k) } 
= 
\frac{\Nhat_k}{N \lambdabar} \left( \frac{1}{\Nhat_k} \sum_{j=1}^{\Nhat_k} \left(c_k(\bx^*_k, \bxihat_{kj}) - \E[c_k(\bx_k^*, \bxi_k)] \right)\right)
\]
Conditional on $\Nhat_k$, 
the sum $ \frac{1}{\Nhat_k} \sum_{j=1}^{\Nhat_k} \left(c_k(\bx^*_k, \bxihat_{kj}) - \E[c_k(\bx_k^*, \bxi_k)] \right)$  is an average of $\Nhat_k$ mean-zero, independent random variables, each of which has magnitude at most $2\Cmax$.  Consequently, by Hoeffding's inequality, with conditional probability at least $1-\frac{\delta}{2K}$,  this term is at most 
\(
\Cmax  \sqrt{ \frac{ 2 \log(4K/\delta) }{ \Nhat_k} }.
\)
Hence, with conditional probability least $1-\frac{\delta}{2K}$, 
\[
\frac{\Nhat_k}{N \lambdabar} \left(  \sum_{j=1}^{\Nhat_k} \left(c_k(\bx^*_k, \bxihat_{kj}) - \E[c_k(\bx_k^*, \bxi_k)] \right)\right)
\leq \frac{\Cmax  \sqrt{ 2 \log(4K/\delta)  }}{N \lambdabar}  \sqrt{\Nhat_k}.
\]
For convenience later on, we can further bound
\(
\sqrt{\frac{\Nhat_k}{N_k}}  \ \leq  \ \sqrt{ 1 + \frac{\abs{\Nhat_k - N_k}}{N_k} }  \ \leq  \ 1 + \frac{\abs{\Nhat_k - N_k}}{N_k}
\),
so that with conditional probability at least $1-\frac{\delta}{2K}$, 
\[
\frac{\Nhat_k}{N \lambdabar} \left(  \sum_{j=1}^{\Nhat_k} \left(c_k(\bx^*_k, \bxihat_{kj}) - \E[c_k(\bx_k^*, \bxi_k)] \right)\right)
\leq \frac{\Cmax  \sqrt{ 2 \lambda_k \log(4K/\delta)  }}{\lambdabar \sqrt N}  \left(1 + \frac{\abs{\Nhat_k - N_k}}{N_k} \right).
\]

For the second term, write 
\[
\abs{\left(\frac{\Nhat_k}{N \lambdabar} - \frac{N_k}{N \lambdabar} \right)\bp_k ^\top \bc_k(\bx^*_k)}
\ \leq \ 
\frac{\Cmax}{N \lambdabar} \abs{ \Nhat_k - N_k}
\ = \ 
\frac{\Cmax \lambda_k }{\lambdabar} \frac{\abs{ \Nhat_k - N_k}}{N_k}
\]

Combining, averaging over $K$ and taking a union bound shows that with conditional probability at least $1-\frac{\delta}{2}$, 
\(
	\abs{\frac{1}{K}\sum_{k=1}^K \frac{\Nhat_k}{N \lambdabar} \bphat_k ^\top \bc_k(\bx^*_k) - \overline Z_K^*}
\)
is at most 
\[
\frac{\Cmax  \sqrt{ 2  \log(4K/\delta)  }}{\sqrt{ N \lambdabar}} 
\ + \ 
\frac{\Cmax  \sqrt{ 2  \log(4K/\delta)  }}{K \lambdabar \sqrt N}   \sum_{k=1}^K \left(\frac{\sqrt{\lambda_k} \abs{\Nhat_k - N_k}}{N_k} \right) + 
\frac{\Cmax \lambda_k }{K \lambdabar}  \sum_{k=1}^K \frac{\abs{ \Nhat_k - N_k}}{N_k},
\]
where we have used Jensen's inequality to bound $\frac{1}{K} \sum_{k=1}^K \sqrt{\lambda_k} \leq \sqrt{\lambdabar}$.
We now convert this conditional probability bound into an unconditional probability bound.  

To this end, notice $\delta > 2K e^{-N_{\min} / 3} \implies N_k > 3 \log (\delta / 2K)$ for every $k$.  Hence, by \cref{lem:PoissonConcentration} and a union bound, we have that with probability at least $1-\delta/2$, 
\begin{equation}
\frac{\abs{ \Nhat_k - N_k}}{N_k}  \leq \sqrt{\frac{ 3 \log (2K/\delta)}{ N_k }} , \quad k =1, \ldots, K,
\end{equation}
simultaneously.  Substituting these upper bounds shows with (unconditional) probability at least $(1-\delta/2)(1-\delta/2) \geq 1-\delta$, we have $\abs{\frac{1}{K}\sum_{k=1}^K \frac{\Nhat_k}{N \lambdabar} \bphat_k ^\top \bc_k(\bx^*_k) - \overline Z_K^*}$ is at most 
\begin{align*}
\frac{\Cmax  \sqrt{ 2  \log(4K/\delta)  }}{\sqrt{ N \lambdabar}}   \ +  \ 
\frac{\Cmax \sqrt{ 6 \log(4K/\delta) \log(2K/\delta) }}{ N\lambdabar }  \ + \ 
\frac{\Cmax \sqrt{3 \log(2K/\delta)} }{  \sqrt {  N \lambdabar }}  ,
\end{align*}
where we have again used Jensen's inequality to bound $\frac{1}{K} \sum_{k=1}^K \sqrt{\lambda_k} \leq \sqrt{\lambdabar}$.  To clean up the bound, notice for $K \geq 1$ and $\delta \leq \frac{1}{2}$, we have $2 \log(K/\delta) \geq 1$.  Collecting constants thus yields, 
\begin{align*}
\frac{6 \Cmax  \sqrt{\log(K/\delta)  } }{\sqrt{ N \lambdabar}}     \ + \ 
\frac{9\Cmax  \log(K/\delta)} {\lambdabar N },
\end{align*}
which completes the proof.  
\hfill \endproof
\end{comment}
%

As a next step, we show that the SAA estimate of performance is uniformly good approximation to the true performance.  To keep the exposition streamlined and proof simple, we make slightly stronger assumptions.  In particular, the assumption of bounded cost functions below is slightly stronger than \cref{asn:bounded}.  We also define
\begin{equation} \label{eq:DefiningDs}
D \equiv \frac{1}{K \lambdabar} \sum_{k=1}^K \lambda_k \text{dim}(\X_k), 
\quad \text{and} \quad
\overline D \equiv \frac{1}{K} \sum_{k=1}^K \text{dim}(\X_k).
\end{equation}
In words, $D$ and $\overline D$ measure the average complexity of the subproblems in terms of the dimension of their feasible regions.  (See also \cref{rem:BetterBoundsVCDim} below for more discussion.)

\begin{lemma}[Relating SAA and True Performance] \label{lem:SAAtoTrue}
Suppose there exists an $R < \infty$ such that $\sup_{\bx_k \in \mathcal X_k} \| \bx_k \| \leq R$ for all $k$ and that 
for each $k$, $\sup_{\bx_k \in \mathcal X_k} \abs{c_{ki}(\bx_k)} \leq C$.  Furthermore, assume \cref{asn:smooth} holds.  Then,  
there exists a universal constant $\const$ such that for any $\max\left(2K e^{-N \lambda_{\min} / 3}, Ke^{-N \lambdabar} \right) < \delta < \frac{1}{2}$, with probability at least $1-\delta$,  
\begin{align*} \hspace{-15pt}
\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k}
\abs{ \frac{\lambda_k}{\lambdabar} \bp_k^\top \bc_k(\bx_k) - \frac{1}{N\lambdabar} \bfmhat_k^\top \bc_k(\bx_k) } 
& \  \leq   \ 
\frac{\const  \Cmax \sqrt{\log(K/\delta) } }{ \sqrt{N \lambdabar}} \cdot 
 \sqrt{ \log\left(\max \left( \frac{R L}{C}, 2 \right) \right) } \cdot \left(\sqrt D + \sqrt{\overline D} \right)
\end{align*}
In particular, this quantity is $O\left( \sqrt\frac{\log(K/\delta)}{ N \lambdabar }\right)$ as $N\lambdabar \rightarrow \infty$ with $K$ fixed.
\end{lemma}


\proof{Proof.}
Define the function $\bcbar_k(\bx) \equiv \frac{\Nhat_k}{N \lambdabar} \bc_k(\bx)$ for all $k$.  Then, the sum in the lemma is bounded above by
\begin{equation} \label{eq:DecomposingInSampleError}
\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k}
\abs{  \bp_k^\top\bc_k(\bx_k) \left(\frac{\lambda_k}{\lambdabar}  - \frac{\Nhat_k}{N \lambdabar} \right) }
\ + \ 
\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k} \abs{ (\bp_k - \bphat_k)^\top \bcbar_k(\bx_k) }
\end{equation}
We first bound each of these sums separately conditional on $\bm{\Nhat}$.  

For the first sum, write 
\[
\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k}
\abs{  \bp_k^\top\bc_k(\bx_k) \left(\frac{\lambda_k}{\lambdabar}  - \frac{\Nhat_k}{N \lambdabar} \right) }
\ \leq \ 
\frac{\Cmax}{K} \sum_{k=1}^K
\abs{  \frac{\lambda_k}{\lambdabar}  - \frac{\Nhat_k}{N \lambdabar} }
 \ = \ 
\frac{\Cmax}{K N \lambdabar} \sum_{k=1}^K \abs{  N_k  - \Nhat_k }, 
\]
where we recall that $N_k \equiv N \lambda_k$.  


%
%
%
%
%
%
%
%
%
%
%
%
%
%

We next bound the second term in \cref{eq:DecomposingInSampleError}.  First fix some $k$.  Notice
\[
\sup_{\bx_k \in \mathcal X_k} \abs{ (\bp_k -\bphat_k)^\top \bcbar(\bx_k) } 
\ = \ 
\sup_{\bx_k \in \mathcal X_k} \abs{ \frac{1}{\Nhat_k} \sum_{j=1}^{\Nhat_k} \cbar_k(\bx_k, \bxihat_{kj}) - \E[\cbar_k(\bx_k, \bxihat_k) ] }.
\]
Conditional on $\Nhat_k$, this is the maximal deviation of an empirical process.  We will analyze it (conditional on $\Nhat_k$) using \cref{thm:pollard} noting here there are now $\Nhat_k$ terms in the sum, not $K$.  

First note that $\frac{\Cmax \Nhat_k}{N \lambdabar} \be$ with $\be \in \mathbb R^{\Nhat_k}$ is a valid envelope with length 
\(
\| \frac{\Cmax \Nhat_k}{N \lambdabar} \be\|  = \frac{\Cmax \Nhat_k^{3/2}}{N \lambdabar}.
\)
Since we have conditioned on $\Nhat_k$, this quantity is a constant.  

We next compute the packing numbers for this process.  To this end, consider an $\frac{C \epsilon}{2 L }$ packing of $\mathcal X_k$.  Since $\mathcal X_k$ is contained in an $\ell_2$-ball of radius $R$, the size of this packing is at most 
\(
 \left(\frac{6 R L }{C \epsilon} \right)^{\text{dim}(\mathcal X_k)}
\)
\citep[Lemma 4.1]{pollard1990empirical}.  
We claim this packing induces a $\frac{C \epsilon \Nhat_k^{3/2}}{2 N \lambdabar}$ covering of our process.  

Indeed, for any $\bx_k \in \mathcal X_k$, let $\by_k$ be the closest element of the packing.  Then, 
\begin{align*}
\left( \sum_{j=1}^{\Nhat_k} \abs{ \cbar_k(\bx_k, \bxihat_{kj}) - \cbar_k(\by_k, \bxihat_{kj}) }^2 \right)^{1/2}
&\ \leq \ 
\frac{\Nhat_k}{N \lambdabar} \left( \sum_{j=1}^{\Nhat_k} \abs{ c_k(\bx_k, \bxihat_{kj}) - c_k(\by_k, \bxihat_{kj}) }^2 \right)^{1/2}
\\
& \ \leq \ 
\frac{L \Nhat_k^{3/2}}{N \lambdabar}  \| \bx_k - \by_k \|_2
\\ 
& \leq \ 
\frac{\Cmax \Nhat_k^{3/2} }{2 N \lambdabar} \epsilon,
\end{align*}
where the penultimate inequality follows because $c_k(\cdot, \bxihat_{kj})$ is $L$-Lipschitz.  Thus, we have a valid $\frac{\Cmax \epsilon \Nhat_k^{3/2}}{2 N \lambdabar}$-covering.  Consequently, the size of an $\frac{\Cmax \epsilon \Nhat_k^{3/2}}{N \lambdabar}$ packing of our process is at most 
\(
 \left(\frac{6 R L }{\Cmax \epsilon} \right)^{\text{dim}(\mathcal X_k)}.
\)

Before invoking \cref{thm:pollard}, we first compute the integral in the definition of $J$.  
Let $\overline L = \max(L, \frac{2\Cmax}{R})$.  Then, 
by \cref{lemma:integral},
\begin{align*}
\int_0^1  \sqrt{ \text{dim}(\mathcal X_k) \log\left(\frac{6 R L}{\Cmax \epsilon} \right) } d\epsilon 
& \ \leq \ \int_0^1  \sqrt{ \text{dim}(\mathcal X_k) \log\left(\frac{6 R \overline L}{\Cmax \epsilon} \right) } d\epsilon 
\\
&\ \leq \ \sqrt{ \text{dim}(\mathcal X_k) } \left( \sqrt{\log\left(\frac{6 R \overline L}{\Cmax} \right) } + \frac{\sqrt \pi}{2}  \right).
\\
&\ \leq \ 
4 \sqrt{ \text{dim}(\mathcal X_k) } \sqrt{  \log\left(\frac{R \overline L}{C} \right) },
\end{align*}
where the last line uses the fact that $R \overline L / C \geq 2$ to simplify and collect constants.  
Hence, 
\(
J \leq 36 \cdot \frac{\Cmax \Nhat_k^{3/2}}{N \lambdabar} \cdot \sqrt{ \text{dim}(\mathcal X_k) } \sqrt{  \log\left(\frac{R \overline L}{C} \right) }.
\)

Finally, applying \cref{thm:pollard} noting again there are $\Nhat_k$ terms in the sum (not $K$), shows that with conditional probability at least $1-\frac{\delta}{2K}$ (conditional on $\Nhat_k$), 
\[
\sup_{\bx_k \in \mathcal X_k} \abs{ (\bp_k - \bphat_k)^\top \bcbar(\bx) } \ \leq \ 
36 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }  \cdot \left(\frac{10K}{\delta}\right)^{1/p} \sqrt{p}  \cdot \frac{\sqrt{\Nhat_k}}{N \lambdabar} \cdot \sqrt{ \text{dim}(\mathcal X_k) }.
\]
Applying a union bound shows that conditional on $\bm{\Nhat}$, with conditional probability at least $1-\delta/2$, 
\[
\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k} \abs{ (\bp_k - \bphat_k)^\top \bcbar_k(\bx_k) }
\ \leq \ 
36 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \cdot \left(\frac{10K}{\delta}\right)^{1/p} \sqrt{p}  \cdot \frac{1}{K} \sum_{k=1}^K \frac{\sqrt{\Nhat_k}}{N \lambdabar} \cdot \sqrt{ \text{dim}(\mathcal X_k) }.
\]

Thus, returning to \cref{eq:DecomposingInSampleError}, we have proven that conditional on $\bm{\Nhat}$, with conditional probability at least $1-\delta/2$, 
\begin{align} \notag
&\frac{1}{K} \sum_{k=1}^K \sup_{\bx_k \in \mathcal X_k}
\abs{ \frac{\lambda_k}{\lambdabar} \bp_k^\top \bc_k(\bx_k) - \frac{1}{N\lambdabar} \bfmhat_k^\top \bc_k(\bx_k)  }
\ \leq \ 
\\ \label{eq:ConditionalBound}
&\quad \quad \frac{\Cmax}{K N \lambdabar} \sum_{k=1}^K \abs{  N_k  - \Nhat_k }
 \ + \ 
36 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \cdot \left(\frac{10K}{\delta}\right)^{1/p} \sqrt{p}  \cdot \frac{1}{K} \sum_{k=1}^K \frac{\sqrt{\Nhat_k}}{N \lambdabar} \cdot \sqrt{ \text{dim}(\mathcal X_k) }.
\end{align}

We now convert this conditional probability bound into an unconditional probability bound.  To this end, 
notice $\delta > 2K e^{-N_{\min} / 3} \implies N_k > 3 \log (2K /\delta )$ for every $k$.  Hence, by \cref{lem:PoissonConcentration} and a union bound, we have that with probability at least $1-\delta/2$, 
\begin{equation} \label{eq:SimultaneousPoissonConcentration}
\abs{ \Nhat_k - N_k} \ \leq \ \sqrt{3N_k \log (2K/\delta) }  \ \leq \ 3 \sqrt{N_k \log(K/\delta)}, \quad \text{simultaneously for all } k =1, \ldots, K.
\end{equation}  
For clarity, in the second inequality we have used $K \geq 1, \delta < \frac{1}{2} \implies K/\delta \geq 2$ to simplify and collect constants.  Moreover, \cref{eq:SimultaneousPoissonConcentration} implies that 
\begin{align} \notag
\frac{\sqrt{\Nhat_k}}{N\lambdabar} 
& \ = \ 
\frac{\lambda_k}{\lambdabar \sqrt{N_k} } \cdot \sqrt{\frac{\Nhat_k}{N_k}}
\\ \notag
& \ \leq \ 
\frac{\lambda_k}{\lambdabar \sqrt{N_k} } \cdot \sqrt{1 + \frac{\abs{\Nhat_k - N_k}}{N_k}}
\\ \notag
&\ \leq \ 
\frac{\lambda_k}{\lambdabar \sqrt{N_k} } \cdot \sqrt{1 + \frac{3 \sqrt{ \log (K/\delta) }} {\sqrt{N_k}}}
\\ \label{eq:RelativePoissonConcentration}
&\ \leq \ 
\frac{\lambda_k}{\lambdabar \sqrt{N_k} } \left( 1 + \frac{3 \sqrt{ \log (K/\delta) }} {\sqrt{N_k}} \right)
\end{align}
Substituting \cref{eq:SimultaneousPoissonConcentration,eq:RelativePoissonConcentration} into \cref{eq:ConditionalBound} shows that with (unconditional) probability at least $(1-\delta/2)(1-\delta/2) \geq 1-\delta$, the sum in the lemma is bounded above by 
\begin{align*}
&\frac{3 \Cmax  \sqrt{ \log (K/\delta) } }{K N \lambdabar} \sum_{k=1}^K \sqrt{N_k }
%
\ + \ 
36 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \cdot \left(\frac{10K}{\delta}\right)^{1/p} \sqrt{p}  \cdot \frac{1}{K} \sum_{k=1}^K \frac{\lambda_k \sqrt{ \text{dim}(\mathcal X_k) }}{\lambdabar \sqrt{N_k} } \left( 1 + \frac{3 \sqrt{\log (K/\delta) }} {\sqrt{N_k}} \right)
\end{align*}
We proceed to ``clean-up" this bound. Notice by Jensen's inequality, $\frac{1}{K} \sum_{k=1}^K \sqrt{N_k} \leq \sqrt{N \lambdabar}$.  Similarly,
%
\begin{align*}
\frac{1}{K} \sum_{k=1}^K \frac{\lambda_k \sqrt{\text{dim}(\X_k)} }{\lambdabar \sqrt{N_k}}
\ = \ 
\frac{1}{\lambdabar \sqrt{N} } \cdot \frac{1}{K} \sum_{k=1}^K \sqrt{\lambda_k \text{dim}(\X_k)}
\ \leq \ 
\frac{1}{\lambdabar \sqrt{N} } \cdot \sqrt{\frac{1}{K} \sum_{k=1}^K \lambda_k \text{dim}(\X_k)}
\ = \ 
\sqrt \frac{ D}{ N\lambdabar },
\end{align*}
%
and
\begin{align*}
\frac{1}{K} \sum_{k=1}^K \frac{\lambda_k \sqrt{ \text{dim}(\mathcal X_k) }}{\lambdabar \sqrt{N_k} } \left( \frac{3\sqrt{\log (K/\delta) }} {\sqrt{N_k}} \right)
 \ = \ 
\frac{3 \sqrt{ \log (K/\delta)}}{N \lambdabar K} \sum_{k=1}^K \sqrt{ \text{dim}(\mathcal X_k) }
 \ \leq \ 
 \frac{3  \sqrt{ \overline D \log (K/\delta)}}{N \lambdabar }.
\end{align*}
Applying these simplifications and collecting constants shows there exists a universal constant $\const_1$, such that with probability at least $1-\delta$, the sum in the lemma is at most
\begin{align*}
& \const_1 \frac{\Cmax \sqrt{\log (K/\delta) } }{ \sqrt{N \lambdabar} } 
\ + \ 
\const_1 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \cdot \left(\frac{10K}{\delta}\right)^{1/p} \sqrt{p}  \left( \frac{\sqrt D}{ \sqrt{N\lambdabar } } + \frac{\sqrt{ \overline D \log (K/\delta)}}{N \lambdabar } \right)
\end{align*}
We can optimize this bound to first order by choosing $p = 2 \log(1/\delta) > 1$.  For this value, we then have for some constant $\const_2$ that the sum in the lemma is at most 
\begin{align*}
& \const_2 \frac{\Cmax \sqrt{\log (K/\delta) } }{ \sqrt{N \lambdabar} } 
\ + \ 
\const_2 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \cdot \sqrt{\log(1/\delta)}  \left( \frac{\sqrt D}{ \sqrt{N\lambdabar } } + \frac{\sqrt{ \overline D \log (K/\delta)}}{N \lambdabar } \right)
\\
&\leq  \
\const_2 \frac{\Cmax \sqrt{\log (K/\delta) } }{ \sqrt{N \lambdabar} } 
\ + \ 
\const_2 \Cmax \sqrt{  \log\left(\frac{R \overline L}{C} \right) }   \left(\sqrt D \sqrt \frac{\log(K/\delta)}{ N\lambdabar } + \sqrt{ \overline D} \cdot \frac{ \log (K/\delta)}{N \lambdabar } \right),
\end{align*}
where we upper bounded $\log(1/\delta) \leq \log(K/\delta)$.  Finally, note that 
\(
\delta > Ke^{-N \lambdabar} \implies \frac{\log(K/\delta)}{N \lambdabar} \leq 1 \implies  \sqrt{ \overline D} \frac{\log(K/\delta)}{N \lambdabar} \leq \sqrt{ \overline D}\sqrt{ \frac{\log(K/\delta)}{N \lambdabar}}.
\)
Applying this last bound and collecting constants proves the lemma.  
\hfill \endproof


We can now prove the main theorem of this section. 
\begin{theorem}[Large-Sample Performance Guarantee for Strongly-Convex Problems.]  \label{thm:LageSample_Smooth}
Suppose there exists an $R < \infty$ such that $\sup_{\bx_k \in \mathcal X_k} \| \bx_k \| \leq R$ for all $k$ and that 
for each $k$, $\sup_{\bx_k \in \mathcal X_k} \abs{c_{ki}(\bx_k)} \leq C$.  Furthermore, assume \cref{asn:smooth} holds.  Then,
there exists a constant $\const$ such that  for any $\delta$ such that $\max\left(2K e^{-N \lambda_{\min} / 3}, Ke^{-N \lambdabar} \right) < \delta < \frac{1}{2}$, we have with probability at least $1-\delta$
\begin{align*}
0 \ \leq \ 
\sup_{\bq \in \Delta_d} \left\{ \Zperf(\alphaLOO_{\bq}, \bq) - Z^* \right\}
&\ \leq \ 
\frac{\const  \Cmax \sqrt{\log(K/\delta) } }{ \sqrt{N \lambdabar}} \cdot 
 \sqrt{ \log\left(\max \left( \frac{R L}{C}, 2 \right) \right) } \cdot \left(\sqrt D + \sqrt{\overline D} \right)
\\
& \quad \ + \ 
\frac{2}{N \lambdabar} \left(\frac{4L^2}{\gamma} + 2C \right).
\end{align*}
In particular, for any choice of anchor $h(\cdot)$, the sub-optimality of the solutions $\bx_k(\alphaLOO_h, h(\bfmhat), \bfmhat_k)$ relative to the full-information optimum is $O\left( \sqrt\frac{\log(K/\delta)}{N \lambdabar} \right)$ as $N\lambdabar \rightarrow \infty$.  Consequently, Shrunken-SAA (with any choice of anchor) achieves full-information optimality in the large-sample limit. 
\end{theorem}
\proof{Proof.}

The first inequality follows because $\overline Z_K^*$ is the full-information optimum.  For the second, 
write the difference as a telescoping sum, 
\begin{subequations}
\begin{align} \label{eq:TrueLOOvsSAALOO}
\Zperf(\alphaLOO_{\bq}, \bq) - \overline Z_K^* 
&\ = \ 
\Zperf(\alphaLOO_{\bq}, \bq) - \ZSAA(\alphaLOO_{\bq}, \bq) 
\\ \label{eq:SAALOOvsSAA0}
& \quad \ + \ 
\ZSAA(\alphaLOO_{\bq}, \bq)  - \ZSAA(0, \bq) 
\\ \label{eq:SAA0vsSAAFullInfo}
& \quad \ + \ 
\ZSAA(0, \bq) - \frac{1}{K } \sum_{k=1}^K \frac{\Nhat_k}{N \lambdabar} \bphat_k^\top\bc_k(\bx^*_k)
\\ \label{eq:SAAFullInfovsFullInfo}
&\quad \ + \ 
\frac{1}{K } \sum_{k=1}^K \frac{\Nhat_k}{N \lambdabar} \bphat_k^\top\bc_k(\bx^*_k)  - \overline Z^*_K.
\end{align}
\end{subequations}
By \cref{lem:SAAOptimizeInsample}, $0$ optimizes the SAA criterion, and hence \cref{eq:SAA0vsSAAFullInfo} is non-positive.  By \cref{lem:LOOToSAA}, \cref{eq:SAALOOvsSAA0} is at most 
\(
\frac{2}{N \lambdabar} \left(\frac{4L^2}{\gamma} + 2C \right).
\)
Finally, both \cref{eq:TrueLOOvsSAALOO} and \cref{eq:SAAFullInfovsFullInfo} can each be upperbounded by 
\[
\frac{1}{K} \sup_{\bx_k \in \X_k} \sum_{k=1}^K \abs{ \left(\frac{\lambda_k}{\lambdabar} \bp_k - \frac{\Nhat_k}{N \lambdabar} \bphat_k \right)^\top \bc_k(\bx_k) }.
\]
This quantity was bounded in \cref{lem:SAAtoTrue}.  Applying that result twice, combining, 
and taking a supremum over $\bq \in \Delta_d$ yields the given bound.  The remaining statements about the performance of Shrunken-SAA with a given anchor follow immediately after noting $h(\bfmhat) \in \Delta_d$.  
\hfill \endproof
%
\begin{remark}[Rate of Convergence]
We note that both SAA and Shrunken-SAA  converge at the same asymptotic rate in $N \lambdabar$ (cf. \cref{lem:SAAtoTrue,thm:LageSample_Smooth}). This might have been guessed already from \cref{lem:LOOToSAA} where we see that Shrunken-SAA is approximately optimal (to order $O_p(1/N)$ ) in the SAA criterion, and, hence, should have a similar rate of convergence.  \Halmos
\end{remark}

\begin{remark}[Improved Bounds for Structured Problems]  \label{rem:BetterBoundsVCDim}
The above bound relies on the complexity measures $D$ and $\overline D$.  One can obtain tighter bounds by making stronger assumptions on the functional form of $c_k(\bx, \bxi)$. Indeed, for many applications, these functions have small pseudo-dimension.  This allows us to construct smaller packings in \cref{lem:SAAtoTrue} which would improve the bound.  The details here are quite standard and omitted (see, e.g., \citealp{pollard1990empirical}). \Halmos
\end{remark}

}

==> Figures/synthDataTrueTable.tex <==
\begin{tabular}{lrrrrrrrr}
  \hline
 & K & Oracle-GM & S-SAA-GM & JS-GM & Oracle-Fixed & S-SAA-Fixed & JS-Fixed & KS \\ 
  \hline
1 &  10 & 14.95 & 12.32 & 9.98 & 12.33 & 7.87 & 5.50 & -8.54 \\ 
  2 &  32 & 9.60 & 7.20 & 3.80 & 6.20 & 3.35 & 0.33 & -11.93 \\ 
  3 &  64 & 10.02 & 8.39 & 4.70 & 7.20 & 6.23 & 0.95 & -11.59 \\ 
  4 & 128 & 12.43 & 11.69 & 5.26 & 9.29 & 9.23 & 1.02 & -11.36 \\ 
  5 & 256 & 12.62 & 12.21 & 4.94 & 9.56 & 9.56 & 0.77 & -10.71 \\ 
  6 & 431 & 12.72 & 12.45 & 5.02 & 9.72 & 9.72 & 0.25 & -10.37 \\ 
  7 & 512 & 12.38 & 12.12 & 5.18 & 9.52 & 9.52 & 0.13 & -10.61 \\ 
  8 & 609 & 12.42 & 12.19 & 5.22 & 9.50 & 9.50 & 0.06 & -10.68 \\ 
  9 & 724 & 12.56 & 12.38 & 5.30 & 9.67 & 9.67 & 0.06 & -10.65 \\ 
  10 & 861 & 12.81 & 12.64 & 5.38 & 9.89 & 9.89 & 0.04 & -10.62 \\ 
  11 & 1024 & 12.62 & 12.46 & 5.35 & 9.68 & 9.68 & 0.00 & -10.79 \\ 
  12 & 1115 & 12.65 & 12.52 & 5.31 & 9.70 & 9.70 & 0.00 & -10.77 \\ 
   \hline
\end{tabular}

